Knowledge-enhanced Visual-Language Pre-training on Chest Radiology Images

While multi-modal foundation models pre-trained on large-scale data have been successful in natural language understanding and vision recognition, their use in medical domains is still limited due to the fine-grained nature of medical tasks and the high demand for domain knowledge. To address this challenge, we propose a novel approach called Knowledge-enhanced Auto Diagnosis (KAD) which leverages existing medical domain knowledge to guide vision-language pre-training using paired chest X-rays and radiology reports. We evaluate KAD on {four} external X-ray datasets and demonstrate that its zero-shot performance is not only comparable to that of fully-supervised models, but also superior to the average of three expert radiologists for three (out of five) pathologies with statistical significance. Moreover, when few-shot annotation is available, KAD outperforms all existing approaches in fine-tuning settings, demonstrating its potential for application in different clinical scenarios.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> content/05-result-nature.tex <==
\section{Results}
The goal of the proposed KAD is to leverage the expert knowledge embedded in a pre-defined knowledge graph, namely, Unified Medical Language System (UMLS)~\cite{bodenreider2004unified}, to improve the vision-language pre-training and facilitate the auto-diagnosis of chest X-ray images. In this section, all self-supervised learning baselines use ResNet50~\cite{he2016deep} as image encoder, 
that are first pre-trained on the MIMIC-CXR~\cite{johnson2019mimic} dataset,
and directly evaluated on three well-established datasets from different perspectives, 
including PadChest~\cite{bustos2020padchest},
NIH ChestX-ray~\cite{wang2017chestx},
and CheXpert~\cite{irvin2019chexpert}.
% including PadChest~\cite{bustos2020padchest} for tail diseases identification, 
% NIH ChestX-ray~\cite{wang2017chestx} for zero-shot and finetuning performance evaluation, CheXpert~\cite{irvin2019chexpert} for comparison with radiologists.
In all cases, the model makes inference by predicting whether the query disease exists in the input image, the difference between zero-shot and finetuning evaluation lies in whether manual annotation is required for training.
\textbf{Note that, all evaluation results from KAD are from zero-shot inference on target dataset unless specified}.
%\weidi{describe the difference .}
%\xiaoman{the difference between zero-shot and supervised?}


\subsection{PadChest}
We evaluate KAD on the diagnosis task in PadChest dataset, 
where the images are labeled with 174 different radiographic findings and 19 differential diagnoses. 
%\xiaoman{How to define the unseen findings? not in the query entity set? 
%but most of the findings are fine-grained categories, take the entity ``tube'' as example, the related findings include ``endotracheal tube'', ``NSG tube'', ``tracheostomy tube''..., should we take them as seen or unseen? }
%\weidi{how many findings are unseen at training time, why this dataset refers to tail diseases identification~(mentioned in above paragraph)}.
The fundamental challenge of PadChest dataset lies in the long-tailed class distribution, as illustrated in Extend Data Fig.~\ref{longtail}, 
where only 21 classes have more than 1000 samples.
%\xiaoman{The flexibility of DQN enables the KAD to directly evaluate arbitrary diseases or radiology findings.}
% zero-shot learning enables the KAD to perform auxiliary diagnoses related to the content found in the knowledge base. 
%\weidi{the above sentence is not clear, reword it, e.g. zero-shot learning ? what do you mean by auxiliary diagnoses ? }
As shown in Fig.~\ref{fig_padchest_auc}, 
KAD outperforms existing SOTA models on most radiographic findings,
and we found that the model achieves an AUC of at least 0.900 on 8 findings and at least 0.700 on 44 out of 57 radiographic findings with at least 50 samples in the PadChest test dataset~($n = 39,053$). 
Extend Data Fig.~\ref{padchest_auc_all1},~\ref{padchest_auc_all2},~\ref{padchest_auc_all3} and~\ref{padchest_auc_all4} includes results on all 193 radiographic findings and diagnoses.
As shown in Table~\ref{padchest_auc},
while comparing the performance with \textbf{fully-supervised} model, 
we observe that KAD significantly outperforms CheXNet on five out of the eight pathologies diagnosis, with AUC of 0.809 ($95\%$ confidence interval (CI) 0.796, 0.822) for atelectasis, 0.916 ($95\%$ CI 0.913, 0.919) for cardiomegaly, 0.910 ($95\%$ CI 0.896, 0.924) for consolidation, 0.966 ($95\%$ CI 0.958, 0.974) for edema and 0.835 ($95\%$ CI 0.829, 0.842) for pneumonia; additionally, KAD demonstrates superior performance than other existing \textbf{self-supervised} visual-language models using image-text pairs, for example, 
AUC $11\%$ higher on pneumothorax than CheXzero~\cite{tiu2022expert}.

\begin{table}[t]
\footnotesize
% \scriptsize
\centering
% \setlength{\tabcolsep}{5.2mm}
\renewcommand{\arraystretch}{1.1}
\caption{Comparison of KAD with SOTA medical image-text pre-training models under \textbf{zero-shot} setting and \textbf{supervised} model~(CheXNet) on the \textbf{PadChest} dataset.}
\rowcolors{1}{LemonChiffon1!20}{LemonChiffon1!20}
\scalebox{0.9}{
\begin{tabular}{p{1.55cm}p{0.9cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.9cm}<{\centering}p{1.2cm}<{\centering}p{1.2cm}<{\centering}}
\rowcolor{LemonChiffon1!50}
\hline
Method & Atelectasis & Cardiomegaly & Consolidation & Edema & Lesion & Pneumonia &  Pneumothorax & No Finding\\
\arrayrulecolor{black}\hline
CheXNet~\cite{rajpurkar2017chexnet}  &  0.794 & 0.908 & 0.840 & 0.939 & \textbf{0.707} & 0.806 & 0.873 & \textbf{0.871}\\
\arrayrulecolor{white}\hline
ConVIRT~\cite{zhang2020contrastive} & 0.527 & 0.508 & 0.531 & 0.559 & 0.496 & 0.567 & 0.562 & 0.497\\
\arrayrulecolor{white}\hline
GLoRIA~\cite{huang2021gloria} & 0.479 & 0.464 & 0.460 & 0.564 & 0.487 & 0.431 & 0.509 & 0.500 \\
\arrayrulecolor{white}\hline
BioVIL~\cite{boecking2022making} & 0.767 & 0.567 & 0.507 & 0.716 & 0.546 & 0.699 & 0.606 & 0.603\\
CheXzero~\cite{tiu2022expert} & 0.798 & 0.898 & 0.871 & 0.961 & 0.651 & 0.789 & 0.766 & 0.755\\
MedKLIP~\cite{wu2023medklip} & 0.768 & 0.863 & 0.823 & 0.766 & 0.672 & 0.769 & 0.754 & 0.612 \\
\arrayrulecolor{white}\hline
KAD~($95\%$ CI) & \textbf{0.809} & \textbf{0.916} & \textbf{0.910} & \textbf{0.966} &  0.657  & \textbf{0.835} & \textbf{0.876} & 0.761 \\
\arrayrulecolor{white}\hline
\rowcolor{LemonChiffon1!50}
 & (0.796, 0.822) & (0.913, 0.919) & (0.896, 0.924) & (0.958, 0.974) & (0.557, 0.757)  & (0.829, 0.842) & (0.839, 0.913) & (0.738, 0.784)\\ 
\arrayrulecolor{black}\hline
\end{tabular}
}
\footnotetext{Note that CheXNet~\cite{rajpurkar2017chexnet} is a fully supervised model trained on PadChest. 
The AUC scores are reported.
Numbers within parentheses indicate $95\%$ CI. The best results are bold.}
\label{padchest_auc}
\end{table}
\vspace{8pt}


%and displays the largest performance gain on pneumothorax compared with best-performing image-text pre-training baseline ().

\begin{figure}[!htb]
\centering
\includegraphics[width=\textwidth]{figure/padchest.pdf}
\caption{
Comparison of KAD with SOTA medical image-text pre-training models under \textbf{zero-shot} setting on unseen radiographic findings in the \textbf{PadChest} dataset.
We evaluate model on the human-annotated subset of the PadChest dataset (n = 39,053 chest X-rays) and mean AUC and $95\%$ CI of KAD are shown for each radiographic finding ($n > 50$) labelled as high importance by an expert radiologist. 
% No labelled samples were seen during training for any of the radiographic findings in this dataset.
KAD achieves an AUC of at least 0.900 on 8 findings  and at least 0.700 on 44 findings out of 57 radiographic findings where ($n > 50$) in the PadChest test dataset (n = 39,053).}
\label{fig_padchest_auc}
\end{figure}


\subsection{ChestXray14}
Fig.~\ref{fig_chestxray} and Extend Data Fig.~\ref{chestxray_auc} and ~\ref{chestxray_ratio} present results of KAD and other approaches on NIH ChestXray14 dataset, where the images are labeled with 14 different diseases, including one unseen class ``fibrosis'', 
not appearing in any of the reports used for training.
%\weidi{how many categories ?}
%\weidi{how many are unseen ?}
% \weidi{hm, the results for this section is in extend data fig. 1, 2, but the previous section is in extend data fig. 4,5,6,7, the order can be optimised ?}
We conduct extensive experiments on both zero-shot and fine-tuning settings, 
in the latter case, we verify the model's performance by varying the percentage of images for fine-tuning. 
As shown in Extend Data Fig.~\ref{chestxray_auc},
KAD achieves the highest performance over all existing self-supervised visual-language models trained with image-text pairs, for instance, it gives an average AUC of 0.786 ($95\%$ CI 0.770, 0.808). For 13 of the 14 pathologies, KAD gets significantly higher AUC than the best-performing baseline. Additionally, in the fine-tuning scenario shown in Extend Data Fig.~\ref{chestxray_ratio}, KAD also demonstrates substantial improvements on all evaluation metrics over the existing approaches.
As we can see, KAD consistently maintains large advantages over other methods under different labeled conditions, and exhibits the largest performance improvements with respect to these baselines when only $1\%$ data is used for training, for example, KAD surpasses ConVIRT by about $13.8\%$, and the widely adopted ImageNet-based pre-training by about $15.2\%$ on average, with largest improvements on hernia~($>29\%$) and edema~($>10\%$), especially under limited supervision.

\begin{figure}[!htb]
\centering
\includegraphics[width=\textwidth]{figure/chestxray_big.pdf}
\caption{Comparison of proposed KAD with SOTA self-supervised baseline models and medical image-text pre-training models on \textbf{ChestXray14} with different ratio of labeled data used for \textbf{fine-tuning}.
AUC, F1 score are reported, and the metrics refer to the macro average on all the diseases.
Note that for fairness, all baselines use the same backbone as the basic image encoder (that is, ResNet50). 
The percentages refer to the percentage of labels used in the training data.}
\label{fig_chestxray}
\end{figure}
\vspace{8pt}

\subsection{CheXpert}
Fig.~\ref{fig_chexpert} and Extend Data Fig.~\ref{chexpert_table} present experimental results from KAD and other image-text pre-training models, 
the performance is compared to three human radiologists on CheXpert test set.
The results show that KAD consistently outperforms existing approaches on the average evaluation scores, demonstrating strong generalisation ability.
When compared with the mean performance of three radiologists,
it is notable that KAD achieves statistically higher mean Matthews Correlation Coefficient (MCC) metric on majority of the competition pathologies.
In particular, on atelectasis (KAD 0.613 ($95\%$ CI 0.567, 0.659) vs. Radiologists 0.548), edema (KAD 0.666 ($95\%$ CI 0.608, 0.724) vs. Radiologists 0.507) and pleural effusion (KAD 0.702 ($95\%$ CI 0.653, 0.751) vs. Radiologists 0.548). On consolidation (Radiologists 0.359 ($95\%$ CI 0.262, 0.444) vs. KAD 0.357), our model is slightly worse, but not statistically significantly.
On the F1 metric, there is no statistically significant difference between the mean performance from KAD 0.647 ($95\%$ CI 0.591, 0.702) and that of the radiologists 0.619 ($95\%$ CI 0.585, 0.642), with only exception on edema, where KAD performs significantly better~(KAD 0.701 ($95\%$ CI 0.647, 0.754) vs. Radiologists 0.583).
%\weidi{should the ablation study be a small, separate section ?}
%\xiaoman{I found the ablation study section is usually given after the detailed introduction of the proposed method (or even without ablation in some papers), so I put it on Sec.~\ref{ablation_study}}
Last but not the least, we provide a thorough ablation study of KAD in Table~\ref{ablation}. More details can be found in the Methods.


\begin{figure}[!tb]
\centering
\includegraphics[width=\textwidth]{figure/chexpert_zeroshot.pdf}
\caption{
Comparisons of proposed KAD with SOTA medical image-text pre-training models and three board-certified radiologists on five competition pathologies in \textbf{CheXpert} dataset. Note that, all models are directly evaluated on CheXpert dataset under \textbf{zero-shot} setting. The AUC, F1 scores and MCC of five pathologies are shown in the plots, where the average and $95\%$ CI are shown. 
Details in Extend Data Fig.~\ref{chexpert_table}. 
%\weidi{Is it possible to make the dots and text just a little bit larger? }
%\xiaoman{Is the current size OK?}
}
\label{fig_chexpert}
\end{figure}
\vspace{8pt}

\begin{table}[!tb]
\footnotesize
\centering
% \setlength{\tabcolsep}{5.2mm}
\renewcommand{\arraystretch}{1.2}
\caption{Ablation study of KAD under \textbf{zero-shot} setting by removing or replacing individual modules.}
\rowcolors{3}{LemonChiffon1!20}{LemonChiffon1!20}
\begin{tabular}{lp{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}}
\hline
\rowcolor{LemonChiffon1!50}
 & \multicolumn{4}{c}{\textbf{ChestXray14}} & \multicolumn{4}{c}{\textbf{CheXpert}} \\ 
\arrayrulecolor{white}\hline
\rowcolor{LemonChiffon1!50}
Methods  & AUC & MCC  & F1  & ACC   & AUC & MCC & F1  & ACC \\ 
\arrayrulecolor{black}\hline
KAD w/o Stage1 & 0.752 & 0.228 & 0.274 & 0.748 & 0.894 & 0.546 & 0.620 & 0.858\\
\arrayrulecolor{white}\hline
KAD w/o entity extraction & 0.772 & 0.212 & 0.262 & 0.814 & 0.897 & 0.568 & 0.638 & 0.872  \\
% \arrayrulecolor{white}\hline
% KAD w/o entity features & 0.751 & 0.242 & 0.290 & 0.780 & 0.878 & 0.571 & 0.671 & 0.812 \\
\arrayrulecolor{white}\hline
KAD w/o DQN & 0.672 & 0.144 & 0.109 & 0.747 & 0.822 & 0.419 & 0.508 & 0.806\\
\arrayrulecolor{white}\hline
KAD ($95\%$ CI) & \textbf{0.789} & \textbf{0.280} & \textbf{0.323 }& \textbf{0.816} & \textbf{0.905 }& \textbf{0.589}& \textbf{0.647} & \textbf{0.875} \\ 
\arrayrulecolor{white}\hline
\rowcolor{LemonChiffon1!50}
 & (0.770, 0.808) & (0.248, 0.312) & (0.294, 0.351) & (0.810, 0.822) & (0.886, 0.924) & (0.534, 0.642) & (0.591, 0.702) & (0.844, 0.906) \\ 
\arrayrulecolor{black}\hline
\end{tabular}
\footnotetext{AUC, MCC, F1 and ACC scores are reported, and the metrics all refer to the macro average on all the diseases.
KAD w/o Stage1 uses PubMedBERT as the text encoder.
KAD w/o entity extraction uses caption for cross-modal contrastive learning.
% KAD w/o entity query use only image features as key or value when training DQN.
KAD w/o DQN only trains the cross-modal contrastive learning part and test like previous image-text pre-training models.
Note that for fairness, all baselines use the same backbone as the basic image encoder (that is, ResNet50). 
Numbers within parentheses indicate $95\%$ CI. The best results are bold.}
% \weidi{simply use Stage1 and Stage2.}}
% \begin{tablenotes}
%  \footnotesize
% \item AUC, MCC, F1 and ACC scores are reported, and the metrics all refer to the macro average on all the diseases.
% KAD w/o Med-KEBERT use PubMedBERT as the text encoder.
% KAD w/o entity extraction use caption for cross-modal contrastive learning.
% % KAD w/o entity query use only image features as key or value when training DQN.
% KAD w/o DQN only train the cross-modal contrastive learning part, and test like previous image-text pre-training models.
% Note that for fairness, all baselines use the same backbone as the basic image encoder (that is, ResNet50). 
% Numbers within parentheses indicate $95\%$ CI. The best results are bold.
% \end{tablenotes}
\label{ablation}
\end{table}


